SVRDA: A Web-based Dataset Annotation Tool for Slice-to-Volume Registration

Background and Objective: The lack of benchmark datasets has impeded the development of slice-to-volume registration algorithms. Such datasets are difficult to annotate, primarily due to the dimensional difference within data and the dearth of task-specific software. We aim to develop a user-friendly tool to streamline dataset annotation for slice-to-volume registration. Methods: The proposed tool, named SVRDA, is an installation-free web application for platform-agnostic collaborative dataset annotation. It enables efficient transformation manipulation via keyboard shortcuts and smooth case transitions with auto-saving. SVRDA supports configuration-based data loading and adheres to the separation of concerns, offering great flexibility and extensibility for future research. Various supplementary features have been implemented to facilitate slice-to-volume registration. Results: We validated the effectiveness of SVRDA by indirectly evaluating the post-registration segmentation quality on UK Biobank data, observing a dramatic overall improvement (24.02% in the Dice Similarity Coefficient and 48.93% in the 95th percentile Hausdorff distance, respectively) supported by highly statistically significant evidence ($p<0.001$).We further showcased the clinical usage of SVRDA by integrating it into test-retest T1 quantification on in-house magnetic resonance images, leading to more consistent results after registration. Conclusions: SVRDA can facilitate collaborative annotation of benchmark datasets while being potentially applicable to other pipelines incorporating slice-to-volume registration. Full source code and documentation are available at https://github.com/Roldbach/SVRDA

==> miscellany/dataset_bullet_points.tex <==
%----------------------------------------------------------------------------------------
%   Indirect Segmentatoin Evaluation
%----------------------------------------------------------------------------------------
\begin{enumerate}
    \item Datasets of nominally healthy volunteers from the UK Biobank (\url{www.ukbiobank.ac.uk}), each of the datasets contained the following
    \item Volumetric scan (neck-to-knee “Dixon technique for internal fat - DICOM” (Data-Field ID 20201)) involved multiple dual echo Dixon VIBE (Volumetric Interpolated Breath-hold Examination) volumes, acquired over the course of 6 min to provide water/fat separated overlapping volumes from the neck to the knees. 
    \item As the 2D image, we used the T1 map derived from the Shortened Modified Look-Locker Inversion recovery (ShMoLLI) scan (named “Pancreas Images - ShMoLLI”, Data-Field 20259). T1 map was computed using a proprietary algorithm from Perspectum Ltd. 
    \item Acquired using Siemens (Siemens Healthineers, Erlangen, Germany) Aera 1.5 tesla (T) scanners
    \item Detailed acquisition parameters for the volume and slice scans have been described previously (cite \url{http://www.nature.com/articles/s41467-020-15948-9} here - see Table 4) 
    \item 3D segmentations of liver and pancreas were generated using automated segmentation methods, namely 3-D U-Net models presented in previous work (cite \url{https://link.springer.com/10.1007/978-3-030-80432-9_21} here). 
    \item 2D segmentations of liver and pancreas were manually delineated by AB (5+ years experience annotating medical images for research). 
    \item \textbf{50?} cases with identified misalignment between the volume and slice data. 
    \item \textbf{Manual selection step} to select cases where both liver and pancreas were visible in the T1 slice? 
\end{enumerate}


%----------------------------------------------------------------------------------------
%   Indirect Segmentatoin Evaluation
%----------------------------------------------------------------------------------------
\begin{enumerate}
    \item Scan-rescan cohort with \textbf{47?} healthy volunteers, where each subject was scanned twice within the same imaging session, after the subject was asked to exit and then re-enter the scanner. 
    \item Volumetric scan: breath-hold, 2-point Dixon T1-weighted VIBE scan, non-quantitative, and covering the entire liver, spleen, pancreas, and kidneys. 
    \item T1 map reconstructed from a ShMoLLI scan targeting the pancreas acquired using similar acquisition parameters to the UK Biobank scans. 
    \item Acquired at three different imaging sites with Siemens scanners: Perspectum Gemini (MAGNETOM Aera 1.5 T), Oxford Centre for Magnetic Resonance (OCMR) (MAGNETOM Prisma 3T) and Chenies Mews Imaging Centre (CMIC) London (MAGNETOM Prisma 3T)
    \item 3D segmentations of liver and pancreas were generated using automated segmentation methods, namely 3-D U-Net models presented in previous work (cite \url{https://link.springer.com/10.1007/978-3-030-80432-9_21} here). 
    \item \textbf{Manual selection step} to select cases where both liver and pancreas were visible in the T1 slice? 
\end{enumerate}
